GPT-in-the-Loop: Adaptive Decision-Making for Multiagent Systems

This paper introduces the "GPT-in-the-loop" approach, a novel method combining the advanced reasoning capabilities of Large Language Models (LLMs) like Generative Pre-trained Transformers (GPT) with multiagent (MAS) systems. Venturing beyond traditional adaptive approaches that generally require long training processes, our framework employs GPT-4 for enhanced problem-solving and explanation skills. Our experimental backdrop is the smart streetlight Internet of Things (IoT) application. Here, agents use sensors, actuators, and neural networks to create an energy-efficient lighting system. By integrating GPT-4, these agents achieve superior decision-making and adaptability without the need for extensive training. We compare this approach with both traditional neuroevolutionary methods and solutions provided by software engineers, underlining the potential of GPT-driven multiagent systems in IoT. Structurally, the paper outlines the incorporation of GPT into the agent-driven Framework for the Internet of Things (FIoT), introduces our proposed GPT-in-the-loop approach, presents comparative results in the IoT context, and concludes with insights and future directions.

==> old/paper_extension.tex <==
**Spotlight on Research Paper: "Integrating Large Language Models into Multiagent Systems for Enhanced Self-Adaptation"**

In the complex world of autonomic computing, self-adaptation is essential for managing multiagent systems (MASs). These systems require sophisticated, direct communication to enhance cooperation, reduce coordination challenges, and adapt dynamically. Our latest research provides an innovative approach, propelling the field further by integrating Large Language Models (LLMs) like GPT-4 into MASs, grounded on the robust MAPE-K model.

In our research, we offer a new paradigm for MAS self-adaptation of autonomous systems leveraging LLM capabilities. This idea presents a significant shift away from traditional models where agents evolve their communication systems over time. We explore the potential of equipping autonomous agents with LLMs from inception and hypothesize a remarkable enhancement in agents' abilities to execute complex tasks and adapt using advanced communication systems.

Our innovative architecture embeds GPT-4, a cutting-edge LLM, within each agent of the MAS. In doing so, we create an environment where every autonomous entity communicates and self-adapts using natural language processing. This methodology, extended from the MAPE-K model, allows for adaptivity in dynamically changing environments, giving our agents advanced communicative capabilities and a unique ability to intelligently react to evolving situations.

To validate our approach, we used a simplified marketplace scenario as a testbed, where autonomous agents, each equipped with an embedded LLM, are tasked with buying and selling books. These agents demonstrated decision-making and emergent behavior, underscoring the potential for self-adaptation.

While the integration of LLMs into MASs presents substantial challenges, such as computational overheads and ethical considerations, we believe it's a promising venture. The use of LLMs in multiagent systems could revolutionize how agents understand, learn from, and interact with their environment and other agents, paving the way for more robust, sophisticated communication, improved adaptability, and enhanced problem-solving capabilities.
